Tools for higher-order network analysis

Networks are a fundamental model of complex systems throughout the sciences, and network datasets are typically analyzed through lower-order connectivity patterns described at the level of individual nodes and edges. However, higher-order connectivity patterns captured by small subgraphs, also called network motifs, describe the fundamental structures that control and mediate the behavior of many complex systems. We develop three tools for network analysis that use higher-order connectivity patterns to gain new insights into network datasets: (1) a framework to cluster nodes into modules based on joint participation in network motifs; (2) a generalization of the clustering coefficient measurement to investigate higher-order closure patterns; and (3) a definition of network motifs for temporal networks and fast algorithms for counting them. Using these tools, we analyze data from biology, ecology, economics, neuroscience, online social networks, scientific collaborations, telecommunications, transportation, and the World Wide Web.

==> CH2-TAB-clique-network-descriptions.tex <==


\begin{table}[htb]
\centering
\dualcaption{Networks for clique scalability experiments}{Although some networks are directed, we undirect all edges.}
\begin{tabular}{l l c c l}
\toprule
Network                    & \# nodes & \# edges \\
\midrule
\dataset{ego-Facebook}     & 4.04K    & 88.2K    \\
\dataset{wiki-RfA}         & 10.8K    & 182K     \\
\dataset{ca-AstroPh}       & 18.8K    & 198K     \\
\dataset{email-EuAll}      & 265K     & 364K     \\
\dataset{cit-HepPh}        & 34.5K    & 421K     \\
\dataset{soc-Slashdot0811} & 77.4K    & 469K     \\
\dataset{com-DBLP}         & 317K     & 1.05M    \\
\dataset{com-Youtube}      & 1.13M    & 2.99M    \\
\dataset{wiki-Talk}        & 2.39M    & 4.66M    \\
\bottomrule
\end{tabular}
\label{tab:networks_cliques}
\end{table}

%\begin{tabular}{l l c c l}
%\toprule
%Network          & description                      & \# nodes & \# edges & source \\
%\midrule
%\dataset{ego-Facebook}     & Facebook friendships             & 4.04K    & 88.2K & \cite{leskovec2012learning,snapnets}                  \\
%\dataset{wiki-RfA}         & Adminship voting on Wikipedia    & 10.8K    & 182K  & \cite{west2014exploiting,snapnets}                    \\
%\dataset{ca-AstroPh}       & author co-authorship             & 18.8K    & 198K  & \cite{leskovec2005graphs,snapnets}                    \\
%\dataset{email-EuAll}      & Emails in a research institution & 265K     & 364K  & \cite{leskovec2005graphs,snapnets}                    \\
%\dataset{cit-HepPh}        & paper citations                  & 34.5K    & 421K  & \cite{gehrke2003overview,leskovec2005graphs,snapnets} \\
%\dataset{soc-Slashdot0811} & Slashdot user interactions       & 77.4K    & 469K  & \cite{leskovec2009community,snapnets}                 \\
%\dataset{com-DBLP}         & author co-authorship             & 317K     & 1.05M & \cite{yang2012defining,snapnets}                      \\
%\dataset{com-Youtube}      & User friendships                 & 1.13M    & 2.99M & \cite{yang2012defining,snapnets}                      \\
%\dataset{wiki-Talk}        & Wikipedia users interactions     & 2.39M    & 4.66M & \cite{leskovec2010governance,snapnets}                \\
%\bottomrule
%\end{tabular}


==> CH2-TKZ-quad_form-common.tex <==
\definecolor{myblue}{RGB}{166,206,227}
\definecolor{mygreen}{RGB}{178,223,138}
\newcommand{\fxpos}{1.25}
\newcommand{\fypos}{-1.5}
\newcommand{\triix}{0.85}
\newcommand{\triiy}{1.35}
\newcommand{\trijx}{0}
\newcommand{\trijy}{0}
\newcommand{\trikx}{1.7}
\newcommand{\triky}{0}

\newcommand{\qfxpos}{1.5}
\newcommand{\qfypos}{-1.65}
\newcommand{\quadix}{0}
\newcommand{\quadiy}{1.7}
\newcommand{\quadjx}{0}
\newcommand{\quadjy}{0}
\newcommand{\quadkx}{1.7}
\newcommand{\quadky}{0}
\newcommand{\quadlx}{1.7}
\newcommand{\quadly}{1.7}

\newcommand{\msize}{18pt}


==> CH2-TXT-abstract.tex <==
 

% Intro sentence
Networks are a fundamental tool for understanding and modeling complex systems
in physics, biology, neuroscience, engineering, and social science.
% State of the field
Many networks are known to exhibit rich, lower-order connectivity patterns that
can be captured at the level of individual nodes and edges.
% Big problem
However, higher-order organization of complex networks---at the level of small
network subgraphs---remains largely unknown.
% Our solution
Here we develop a generalized framework for clustering networks based on
higher-order connectivity patterns.  This framework provides mathematical
guarantees on the optimality of obtained clusters and scales to networks with
billions of edges.  The framework reveals higher-order organization in a number
of networks including information propagation units in neuronal networks and hub
structure in transportation networks.
% Concluding sentence
% This sentence needs to start with our
Results show that networks exhibit rich higher-order organizational structures
that are exposed by clustering based on higher-order connectivity patterns.


==> CH4-FIG-intro2.tex <==
\definecolor{myred}{RGB}{228, 26, 28}
\definecolor{myblu}{RGB}{55, 126, 184}
\definecolor{mypur}{RGB}{152, 78, 163}
\begin{figure}[tb]
\centering
\includegraphics[width=\columnwidth]{CH4-FIGFILE-intro2.pdf}
\dualcaption{Example execution of \cref{alg:general} for counting instances of the
  $\delta$-temporal motif $M$ and network in \cref{fig:intro1}}{%
%
Each column shows the value of counters at the end of the for loop that
processes temporal edges.  Color indicates change in the variable: incremented
(\textcolor{myblu}{blue}), decremented (\textcolor{myred}{red}),
incremented and decremented (\textcolor{mypur}{purple}), or no change
(black).  At the end of execution, $\counts[(a,b)(a,c)(c,a)] = 2$ for the two
instances of the temporal motif $M$ with center node $a$.  Here we only show the
counters needed to count $M$; in total, \cref{alg:general} maintains 39 total
counters for this input edge sequence, 25 of which are non-zero.
%
}
\label{fig:intro2}
\end{figure}


==> CH4-FIG-similar-pca.tex <==


\begin{figure}[tb]
\centering
\includegraphics[width=0.6\columnwidth]{CH4-FIGFILE-similar_datasets_PCA_variance_updated}
\dualcaption{Temporal networks from the same domain have similar
  motif counts}{%
%
We plot the percentage of explained variance of relative counts of collections
of datasets plotted as a function of the number of principal components.  In
datasets from the same domain, 90\% of variance is explained with fewer
components.
%
}
\label{fig:similar_counts_PCA}
\end{figure}

